Contrast and Classify: Training Robust VQA Models

Recent Visual Question Answering (VQA) models have shown impressive performance on the VQA benchmark but remain sensitive to small linguistic variations in input questions. Existing approaches address this by augmenting the dataset with question paraphrases from visual question generation models or adversarial perturbations. These approaches use the combined data to learn an answer classifier by minimizing the standard cross-entropy loss. To more effectively leverage augmented data, we build on the recent success in contrastive learning. We propose a novel training paradigm (ConClaT) that optimizes both cross-entropy and contrastive losses. The contrastive loss encourages representations to be robust to linguistic variations in questions while the cross-entropy loss preserves the discriminative power of representations for answer prediction. We find that optimizing both losses -- either alternately or jointly -- is key to effective training. On the VQA-Rephrasings benchmark, which measures the VQA model's answer consistency across human paraphrases of a question, ConClaT improves Consensus Score by 1 .63% over an improved baseline. In addition, on the standard VQA 2.0 benchmark, we improve the VQA accuracy by 0.78% overall. We also show that ConClaT is agnostic to the type of data-augmentation strategy used.

==> sections/intro.tex <==
\section{Introduction}

\begin{figure}[t!]
\centering
\includegraphics[width=0.9\linewidth]{figures/AAAITeaserv6.png}
\caption{We make VQA model robust to question paraphrases using a training paradigm ConCAT that alternately minimizes contrastive and cross-entropy loss. Contrastive learning step pulls representations of positive samples corresponding to paraphrased questions closer together while pushing those with different answers farther apart. Cross-entropy step makes these representations discriminative to help model answer visual questions accurately.}
\label{fig:teaser}
\end{figure}

% \item VQA models are inconsistent and brittle

% \item Explain what is inconsistency and why it matters. [reliablity etc.]

Visual Question Answering (VQA) refers to the task of automatically answering free-form natural language questions about an image. For VQA systems to work reliably when deployed in the wild for applications such as assisting visually impaired users, they need to be robust to different ways a user might ask the same question. 
For example, VQA models should produce the same answer for two paraphrased questions – ``What is in the basket?'' and ``What is contained in the basket?'' since their semantic meaning is same. While significant progress has been made towards building more accurate VQA systems, these models are still sensitive to minor linguistic variations in the input question. 


% VQA model <Q1> vs <parphrased Q1> result in two entirely different answers whereas to us the both mean the same thing. 
% In order to benchmark progress of VQA models previous work \cite{} collected human rephrasings on the subset original VQA 2.0 validation set. 


% \item Explain how present-day VQA models learn joint V+L representations
% \item Explain how existing approaches tackle robustness in VQA

To make VQA systems more robust, % to small linguistic variations, 
existing approaches~\cite{shah2019cycle,tang2020semantic} train state-of-the-art VQA systems~\cite{jiang2018pythia} on augmented data which includes different variations of the input question. For instance, VQA-CC~\cite{shah2019cycle} use a visual question generation (VQG) model to generate paraphrased question given an image and an answer. %where as ~\cite{tang2020semantic} uses back-translation to produce question rephrasings. 
These models fuse image and question features into a joint vision and language (V+L) representation followed by a standard softmax classifier to produce answer probabilities. The models are optimized by minimizing the standard cross-entropy loss. \CE/ loss treats every image-question pair independently and fails to exploit the information that some questions in the augmented dataset are paraphrases of each other.

%The VQA system is jointly trained to produce the same answer for both the original and the generated question. Since, the VQG model is trained on the same training corpora on which the VQA model was trained, these models tend to overfit to the style of questions in the training dataset. 
% On the other hand, ~\cite{tang2020semantic} 
% % encourages model generalization to paraphrased questions by augmenting
% augment the dataset with questions generated via back-translation. Back translation involves translating an input sentence from one language to another and then using a separate independent translator to translate it back into the original language. Back-translation preserves the semantic meaning of the question but generates syntactically diverse question paraphrases.
% semantically equivalent adversarial examples that fool the VQA model to produce a different answer.

%Furthermore, VQA-CC follow the canonical style of training VQA models and do not fully exploit the augmented data. These models fuse image and question features into a joint vision and language representation followed by a standard softmax classiﬁer to learn a probability distribution over the answers. Intuitively, the learned vision and language representations should have high intra-class similarity i.e. image-question pairs that have the same answer should be closer together. Simultaneously, these representations should have high inter-class separability i.e. imagequestions pairs having different answers should be far apart. However, previous works (Liu et al. 2016) have shown that using the standard \CE/ loss does not explicitly encourage intra-class similarity and inter-class separability.

% We overcome this limitation by using a contrastive loss InfoNCE~\cite{Oord2018RepresentationLW} that encourages joint V+L representations obtained from the question and its paraphrase to be closer together while pulling apart the V+L representations for questions with different answers.

We overcome this limitation by using a contrastive loss InfoNCE~\cite{Oord2018RepresentationLW} that encourages joint V+L (Vision and Language) representations obtained from samples whose questions are paraphrases of each other to be closer while pulling apart the V+L representations of samples with different answers. Since we operate in a supervised setting, we choose Supervised Contrastive Loss (SCL)~\cite{Khosla2020SupervisedCL} which extends InfoNCE to utilize label information by bringing samples from the same class together. We introduce a variant of the SCL which emphasizes on rephrased image-question pairs over pairs that are entirely different but have the same answer.
% \ha{We introduce a variant of the SCL loss (\lsscl/) which assigns higher weight to augmented positive samples (rephrasings in our case) over intra-class positive samples (that have the same answer).} 
Our proposed training paradigm (\concat/) alternately minimizes the SCL with cross-entropy loss to learn better vision and language representations as shown in Fig.\ref{fig:teaser}. Minimizing the contrastive loss encourages representations to be robust to linguistic variations in questions while the cross-entropy loss preserves the discriminative power of the representations for answer classification. Instead of pretraining with \SCL/ loss, then fine-tuning with cross-entropy loss as in~\cite{Khosla2020SupervisedCL}, we find that minimizing the two losses alternately by constructing loss-specific mini-batches helps learn better representations. For the contrastive loss, we carefully curate these loss-specific mini-batches by sampling various types of negatives and positives given a reference.

We show the efficacy of our training paradigm across two rephrasing or data-augmentation  strategies. Using rephrasings obtained from a VQG model proposed in~\cite{shah2019cycle}, our approach outperforms a baseline that simply treats these rephrasings as additional samples and ignores the link between question and its paraphrases. We noticed that VQG model fails to produce a diverse set of rephrasings for a question and experiment with using Back-translation to obtain question rephrasings. \BT/ \cite{edunov2018understanding} involves translating an input sentence from one language to another and then translating it back into the original language using a pair of machine translation models (e.g. \texttt{en-fr} and \texttt{fr-en}). \BT/ preserves the semantic meaning of the question but generates syntactically diverse question paraphrases. Utilizing the publicly available collection of neural machine translation models in HuggingFace~\cite{Wolf2019HuggingFacesTS}, we generate 88 rephrasings of a question using MT model pairs for 88 different languages. We use a sentence similarity model \cite{reimers2019sentencebert} to filter irrelevant rephrasings and obtain 3 rephrasings per original question of VQA v2.0 dataset \textit{without} any manual supervision.

We perform ablations to show that optimizing the contrastive loss and \ce/ loss alternately helps compared to jointly optimizing them or pretraining with contrastive loss and then finetuning with \ce/ approach in ~\cite{Khosla2020SupervisedCL}. We also show that curating batches with  our proposed negative sampling strategy further boosts performance. 
On the VQA Rephrasings benchmark which measures the model's answer consistency across several rephrasings of a question, \concat/ improves Consensus Score~\cite{shah2019cycle} by 1.63\% over an improved baseline. In addition, on the standard VQA 2.0 benchmark, we improve the VQA accuracy by 0.78\% overall. It is also worth noting that under our training paradigm (ConCAT), VQA models show better performance than existing approaches across both the aforementioned data-augmentation strategies.

% % \item Summarize Contributions [-Alternate SCL -Hard Mining -BT data?]

% % Overall we improve --- on VQA-Reprasings and --- on VQA 2.0 validation set. Our contributions are as follows: --- \yk{Expand more}
% To summarize, we make the following contributions.
% \begin{itemize}
%     \item We propose a novel training paradigm that involves alternate training of contrastive and \CE/ losses to learn joint vision and language representations that are robust to linguistic variations in input questions. 
%     \item We automatically collect a large-scale dataset of X paraphras questions to complement the original VQA dataset using back translation with publically available neural machine translation models. 
%     \item We emperically show that our proposed approach improves consistency score and VQA scores on the VQA-Rephrasings and VQA2.0 dataset respectively across a variety of data augmentation techniques. 
% \end{itemize}



==> sections/method.tex <==
%% make figure
\begin{figure*}[t!]
  \centering
  \includegraphics[width=\textwidth]{figures/Approachv2.pdf}
  \caption{Dummy caption}
  \label{fig:approach}
\end{figure*}


\section{Preliminaries}
% In this section, we first introduce notations and expand on our VQA architecture that jointly learns V+L representations. 
% Next, we present our modified formulation of Supervised Contrastive Loss \cite{Khosla2020SupervisedCL} 
% for our use case. Finally, expand on the details of our alternate training paradigm and mini-batch creation
% process for the contrastive loss. 
% In this section, we introduce the VQA task and the typical cross entropy training of the VQA models. We then recap contrastive learning and the recently proposed Supervised Contrastive Learning (\SCL/) \cite{Khosla2020SupervisedCL} loss.
In this section, we introduce the VQA task and the typical cross entropy training of the VQA models. We then recap contrastive methods for learning representations~\cite{chen2020simple} and the recently proposed Supervised Contrastive Learning (\SCL/) \cite{Khosla2020SupervisedCL} setup.
%discuss our proposed training paradigm to train VQA models which are robust to minor linguistic variations in the questions. We start with an overview of the VQA dataset and how to augment the dataset with question rephrasings. We then introduce our training paradigm that involves alternately optimizing cross-entropy loss with our variant of the Supervised Contrastive Learning (SCL)~\cite{Khosla2020SupervisedCL} loss. Finally, we describe how carefully curating batches for the two losses can help learn more robust VQA models. 

\textbf{VQA.} 
The task of Visual Question Answering (VQA)~\cite{vqa,goyal2016making} involves predicting answer $a$ for a question $q$ asked about an image $v$. In the VQA dataset $\mathcal{X}$, an instance $x$ can be represented with a triplet consisting of an image $v$, a question $q$ and its ground-truth answer $a$ represented as $(v, q, a), \ \forall \ x \in \mathcal{X}$. \am{Alternate start to VQA para: Visual Question Answering (VQA)~\cite{vqa,goyal2016making} involves answering free-form, open-ended natural language questions for a given image. To be specific, given a VQA dataset $\mathcal{X}$ with each sample $x \in \mathcal{X}$, a triplet consisting of an image $v \in \mathcal{V}$ , a question $q \in \mathcal{Q}$ and its ground-truth answer $a \in \mathcal{A}$ represented as $(v, q, a)$, the task of Visual Question Answering (VQA)~\cite{vqa,goyal2016making} is to learn a model $f : {\mathcal{V} \times \mathcal{Q}} \rightarrow \mathcal{A}$ which could yield a natural language answer for a given visual question.
} 
A typical VQA model $f$ \am{Seems like figure notations are running totally different from text notations. $f$ is feature extractor in figure. We should fix this.}takes image and question as input and outputs a joint vision and language (V+L) $d_h$-dimensional representation $\bm h \in \mathcal{R}^{d_h}$ \am{$d_h$ sounds odd. Fix: outputs a joint vision and language (V+L) representation $\bm h \in \mathcal{R}^{d}$} using a multi-modal attention network $f^{mmt}$:
% $$\bm{h} = f^{mmt}(v, q; \theta^{mmt})$$
$$\bm{h} = f^{mmt}(v, q)$$


The V+L representations $\bm{h}$ is used to predict a probability over the answer space \am{answer space $\mathcal{A}$} via a simple softmax classifier $f^{c}(\bm h;\theta^c)$ parametrized by $\theta^c$ to learn a probability distribution over the answer space $\mathcal{A}$ via:
\am{Too long sentence with repetition, "to predict a probability", "to learn a probability". Suggestion: The V+L representations $\bm{h}$ is used to predict a probability distribution over the answer space $\mathcal{A}$ with a simple softmax classifier $f^{c}(\bm h)$ which is learned via:}

$$p_{\theta}(a|v,q) = \frac{\exp(f^c(\bm h)[a])}{\sum_{a'\in \mathcal{A}}\exp(f^c(\bm h)[a'])}$$
\begin{equation}
\begin{aligned}
        % \bm h &= f^{mmt}(v,q)\\
        % \mathcal{L}_{ce} = \min_{\theta} &-\mathbb{E_{\mathcal{X}}}[\log p_{\theta}(a|v,q)]
        \min_{\theta}~ \mathcal{L}_{ce} =  &-\mathbb{E_{\mathcal{X}}}[\log p_{\theta}(a|v,q)]
\end{aligned}
\end{equation}
where $f^c(f^{mmt}(v, q))[a]$ indicates the logit corresponding to the $a^{th}$ label and $\theta=[\theta^{mmt}, \theta^{c}]$ is a list of all the parameters of the VQA model $f^{vqa} = f^c \circ f^{mmt}.$ 
\am{$f^c(\bm h)[a]$  indicates the logit corresponding to the answer $a$. Remove theta from all equations.}

\textbf{Contrastive Learning.} Recent works in vision \cite{chen2020simple} have used contrastive losses to bring representations of two augmented views of the same sample\am{image} (called positives) closer together while pulling apart the representations of two different samples\am{images} (called negatives). %Following recent works in contrastive learning \cite{chen2020simple,Khosla2020SupervisedCL}, we want to bring joint V+L representations obtained from  the question and its paraphrase to be closer together while pulling apart the V+L representations for questions with different answers. 
\yk{Try to rephrase the next statement better} In this, the obtained representation $h = f_\theta(x)$ is projected  into a $d_p$-dimensional hyper-sphere normalized vector $z = g(h) \in \mathcal{R}^{d_p}$. Next, given a mini-batch of size $N$, the representations are learned by minimizing the InfoNCE~\cite{Oord2018RepresentationLW} loss which operates on representations belonging to pair of positives $(z_i,z_j)$ and $N-1$ negatives $(z_i,z_k), k\in \{1...N\}, k\neq i$ as below:

\begin{equation}
\label{eq:nce_loss}
    \mathcal{L}_{nce}^{ij} = -\log \frac{\exp(\Phi(\bm z_i, \bm z_j)/\tau)}{\sum_{k=1}^{N} \mathbbm{1}_{k \neq i}\exp(\Phi(\bm z_i, \bm z_k)/\tau)}~,
\end{equation}
\am{not sure why do we need superscript $ij$ over the NCE loss term. We are not going to use this anywhere. InfoNCE paper defines loss over a batch which is consistent with what we are saying here. $ij$ is also a bit weird to write in loss superscript.}
where $\mathrm{\Phi}(\bm u,\bm v) = \bm u^\top \bm v / \lVert\bm u\rVert \lVert\bm v\rVert$ denotes a similarity function between $\bm u$ and $\bm v$ and $\tau > 0$ is a scalar temperature parameter.

A generalization of InfoNCE loss to handle more than one positive-pair was proposed by \cite{Khosla2020SupervisedCL} called Supervised Contrastive Loss (\SCL/). Given a reference sample $x$, SCL uses class-label information to form a set of positives $\mathcal{P}(x)$. More specifically, $\mathcal{P}(x)$ contains augmented views of the sample $x$ and samples with same ground truth as $x$. For a minibatch with $N$ samples the \SCL/ loss then becomes:
% The \SCL/ loss given a reference sample $x_i$ and corresponding set of positives denoted by $\mathcal{P}(x_i)$ 
% The set of positives $\mathcal{P}(x_i)$ also contain augmented views of the sample $x_i$ since they also have the same ground-truth label as $x$.
\begin{equation}
\mathcal{L}_{scl}^{i} = -\sum_{p=1}^{\vert \mathcal{P}(x_i) \vert} { \log \frac{\exp(\Phi(\bm z_i.\bm z_p)/\tau)}{\sum_{k=1}^{N}{\mathbbm{1}_{k \neq i}
\cdot \exp(\Phi(\bm z_i.\bm z_p)/\tau)}}} \label{eq:scl_i}
\end{equation}

\begin{equation}
\mathcal{L}_{scl} = \sum_{i = 1}^{N}{\frac{\mathcal{L}^{i}_{scl}}{\vert \mathcal{P}(x_i) \vert}} 
 \end{equation}

Overall, \SCL/ tries to bring the representation of samples $x_i$ and $\hat{x}_i \in \mathcal{P}(x_i)$ closer together compared to representations of samples that have different ground-truth label.

\section{Approach}
We now describe our proposed training paradigm, ConCAT, that uses contrastive learning along with cross-entropy training to learn VQA models robust to question rephrasings. 
 
\textbf{Contrastive Learning in VQA.} For a sample $x = (v, q, a), \ \forall \ x \in \mathcal{X}$, let's denote a set of paraphrases for question $q$ by $\mathcal{Q}(q)$ and the corresponding 
set of VQA triplets: 
$$\mathcal{P}^r(x) = \{(v, q_r, a) \ |\  \forall q_r \in \mathcal{Q}(q)\}.$$
\am{this definition of rephrasings set is incomplete, not clear where $v$ and $a$ come from. Also, $q$ does not appear anywhere in the equation.}

We also define the set of all samples with the same ground truth as $x$ by: 
$$\mathcal{P}(x) = \{\hat{x}  = (\hat{v}, \hat{q}, \hat{a}) \mid \hat{a} = a, \forall \hat{x} \in \mathcal{X}\}.$$ 

The set of all paraphrases $\mathcal{P}^r(x)$ is a subset of all positives $\mathcal{P}^r(x) \subset \mathcal{P}(x)$ as all question rephrasings have the same answer for a given image but not all questions with the same answer are paraphrases of each other. \yk{Simplify next statement} We augment the VQA dataset $\mathcal{X}$ with a set of triplets $\mathcal{P}^r(x)$ formed using multiple paraphrases of a question belonging to all the samples in $\mathcal{X}$. We denote the augmented dataset with $\mathcal{X}^{aug}$. We generate these paraphrases
either by using \BT/~\cite{edunov2018understanding} or a \VQG/ model~\cite{shah2019cycle} .

Ideally, we would like our VQA model to produce the \textit{same and correct} answer for a question and its paraphrase on the same input image \ie: 
$$f^{vqa}(v, q) = f^{vqa}(v, q_r) = a\ \forall q_r\in Q^r(q).$$

This motivates us to map joint V+L representations of an original and paraphrased sample closer to each other. Moreover, since we operate 
in a supervised setting, following learning~\cite{Khosla2020SupervisedCL} we also try to bring the joint representations for the questions with the same answer closer together while pulling apart the representations of questions with different answers. 

Using $\mathcal{P}(x_i)$ in Eq\eqref{eq:scl_i} will treat paraphrased question and question with the same answer equally. 
% Similar to using just cross-entropy loss on the augmented dataset, 
SCL loss fails to emphasize the link between question and its paraphrase, to overcome this, we propose a variant of the SCL loss in Eq\eqref{eq:sscl_i} which assigns higher weight to augmented positive samples $\mathcal{P}^{r}(x)$ (question paraphrases) over intra-class positive samples $\mathcal{P}(x) - \mathcal{P}^{r}(x)$ (questions that have the same answer). Formally, we introduce a scaling factor $\alpha_{ip}$ in the SCL loss (Eq\eqref{eq:scl_i}) for a sample $x_i$ as follows: 
\begin{equation}
\mathcal{L}_{sscl}^{i} = -\sum_{p=1}^{\vert \mathcal{P}(x_i) \vert} {\alpha_{ip} \cdot \log \frac{\exp(\Phi(\bm z_i.\bm z_p)/\tau)}{\sum_{k=1}^{N}{\mathbbm{1}_{k \neq i}
\cdot \exp(\Phi(\bm z_i.\bm z_p)/\tau)}}} \label{eq:sscl_i}
\end{equation}
\begin{equation}
% \mathcal{L}_{sscl} = \sum_{i = 1}^{N}{\frac{\mathcal{L}^{i}_{scl}}{\sum_{p=1}^{\vert \mathcal{P}(x_i) \vert}\alpha_{ip}}} 
\mathcal{L}_{sscl} = \sum_{i = 1}^{N}{\frac{\mathcal{L}^{i}_{scl}}{\sum_{p}\alpha_{ip}}} 
\end{equation}

The scaling factor $\alpha_{ip}$ assigns a higher weight $s>1$ to positive samples corresponding to question paraphrases compared to other intra-class positives. Intuitively, because of the higher weight, the loss will penalize the model strongly if it fails to bring 
the representations of a question and its paraphrase closer. Formally, we define $\alpha_{ip}$ as: 
\begin{equation}
\alpha_{ip} = 
\begin{cases}
    s& \text{if } x_p \in \mathcal{P}^{r}(x_i),   \\
    1,              & \text{otherwise}
\end{cases}
\end{equation}

\subsection{Alternate Training}
In contrast with \cite{Khosla2020SupervisedCL} who pretrain their network using \lscl{} and finetune it on cross-entropy \lce{}, we train our model by alternating between \lsscl{}  and the cross-entropy \lce{}  iterations. The benefit of our  approach is twofold: First, we have a single-stage training as compared to two-stage training in \cite{Khosla2020SupervisedCL}.
Second, training alternately allows us to curate batches with multiple-positives and hard-negatives (see \ref{ssec:batchmining} \yk{todo}) for \lsscl{} that helps to further boost the performance without affecting the \lce{} training. 
% The benefit of our approach is twofold: The main advantage of alternate training compared to two-stage training in \cite{Khosla2020SupervisedCL} is that it allows us to curate loss-specific batches with multiple-positives and hard-negatives (see \ref{ssec:batchmining} for \lscl{} that further boosts the performance without affecting the \lce{}.  
Our training paradigm is summarized in Algorithm \ref{alg:main}. Specifically, given $N_i$ total training iterations, we update our model with \lscl{} after every $N_{ce}$ updates with \lce{} where $N_{ce}$ is a hyper-parameter. Our overall loss can be written as: 
\begin{equation}
    \label{loss:vqa}
    \mathcal{L}_{vqa} = \mathbbm{1}_{n\Mod{N_{ce}} = 0} \cdot \mathcal{L}_{sscl} + \mathbbm{1}_{n\Mod{N_{ce}} \neq 0} \cdot \mathcal{L}_{ce}
\end{equation} 
\begin{algorithm}[t]
\caption{\label{alg:main} Alternate Optimization with \lsscl{} and \lce{}}
\begin{algorithmic}
    \STATE \textbf{input:} steps $N_i$; constant $N_{ce}$; train data $\mathcal{X}$; networks $f,g$
    % \STATE \textbf{function} CURATE($N_r$, $\mathcal{X}$, $\tau$, $\bm \alpha$)
        % \STATE $~~~~$\textcolor{gray}{\# intialize batches}        
        % \STATE $~~~~$ $\mathcal{B} = \phi, \mathcal{B}_r = \phi$
        \STATE $~~~~$ \textbf{for all} $i\in \{1, \ldots, N_i\}$ \textbf{do}
        \STATE $~~~~~~~~$ $\mathcal{B} = \phi, \mathcal{L} = \phi$

        \STATE $~~~~~~~~$ \textbf{if} $i \Mod{N_{ce}} = 0$ \textbf{do}
        \STATE $~~~~~~~~~~~$\textcolor{gray}{\# scl iteration}        
        \STATE $~~~~~~~~~~~$ $\mathcal{B}=$ CURATE($N_r$, $\mathcal{X}$, $\bm w$); $\mathcal{L}=$ \lscl{}
        % \STATE $~~~~~~~~$ $\mathcal{L}= \mathcal{L}_{scl}$

        \STATE $~~~~~~~~$ \textbf{else} \textbf{do}
        \STATE $~~~~~~~~~~~$\textcolor{gray}{\# ce iteration}
        \STATE $~~~~~~~~~~~$ sample $\mathcal{B} \!\sim\! \mathcal{X}$; $\mathcal{L}=$ \lce{}
        \STATE $~~~~~~~~$ update $f(.),g(.)$ networks to minimize $\mathcal{L}$ over $\mathcal{B}$
        
    \STATE \textbf{return} network $f(.)$; throw away $g(.)$
\end{algorithmic}
\end{algorithm}

\subsection{Negative Types and Batch Creation} \label{ssec:batchmining}
Any contrastive loss including SCL operates with multiple negative samples. 
% We define a set of negatives $\mathcal{N}(x) \subseteq \mathcal{X}^{aug}$ for any reference sample $x \in \mathcal{X}^{aug}$ as a collection of samples that have a different answer than the sample:
For a given reference sample $x = (v, q, a), \ \forall \ x \in \mathcal{X}^{aug}$, we define a corresponding set of negatives as samples with ground truth different than the reference $x$:
\begin{equation*}
    \mathcal{N}(x) = \{\bar{x} = (\bar{v}, \bar{q}, \bar{a}) \mid  \bar{a}\neq a, \bar{x} \in \mathcal{X}^{aug}\}.
\end{equation*}


% The minibatches for \lscl{} in~\cite{Khosla2020SupervisedCL} are created by first sampling a set of anchor samples and the corresponding positive pairs. For every sample, other samples in the minibatch with a different ground-truth label is considered negative. 

We carefully curate batches for \lsscl{} by sampling different types of negatives. For this, we classify a negative pair $({x}, \bar{x})$ into one of three negative categories from $\mathcal{T}=$ \texttt{[que, img, rand]} via a mapping function $\Omega:{\mathcal{X} \times \mathcal{X}} \rightarrow \mathcal{T}$: such that:
\begin{equation}
\Omega({x}, \bar{x}) = 
\begin{cases}
    \texttt{img}  & \text{if } v = \bar{v}  \\
    \texttt{que}  & \text{if } sim(q, \bar{q}) > \epsilon  \\
    \texttt{rand} &  \text{else}
\end{cases}
\end{equation}

We now partition $\mathcal{N}(x)$ in three mutually exclusive subsets $\mathcal{N}^t(x), t \in \mathcal{T}$ defined as:
\begin{equation}
    \mathcal{N}^t(x) = \{\bar{x} \mid \Omega({x}, \bar{x}) = t, \forall \bar{x} \in \mathcal{N}(x) \}
\end{equation} 

\begin{itemize}
    \item \textbf{Image Negatives}, ($ \mathcal{N}^{\texttt{img}}(x)$): Image negatives ($\bar{x}^{\texttt{img}}$) are samples 
    that have same image as the reference ($x$) but different answer. Since VQA dataset has multiple questions ($\sim$ 5.4) per image, finding image negatives is trivial. 
    \item \textbf{Question Negatives}, ($ \mathcal{N}^{\texttt{que}}(x)$):  Question negatives $(\bar{x}^{\texttt{que}})$ are samples 
    with similiar questions and different answers. We measure the similarity between the questions by computing their cosine distance in the vector space of the Sentence-BERT \cite{reimers2019sentencebert} model. We denote this by $sim(q, \bar{q}^{\texttt{~que}}) > th$. 
    % The similarity between the questions is computed by using representations from Sentence-BERT introduced by \cite{reimers2019sentencebert}.
    \item \textbf{Random Negatives}, ($ \mathcal{N}^{\texttt{rand}}(x)$): Random negatives $(\bar{x}^{\texttt{rand}})$ are samples do not fall under either Image or Question negative categories. \\
\end{itemize}

\textbf{Batch Curation for \lsscl{}}: As described in Algorithm~\ref{alg:batch}, we start by filling our batch with triplets of reference $x_i$, a intra-class positive $\hat{x_i}^{p}$ and a negative sample $\bar{x_i}^{t}$ of type $t$. The negative type $t$ is sampled from a categorical distribution $Cat(T\vert\bm w)$ where $\bm w = (w^{\texttt{img}}, w^{\texttt{que}}, w^{\texttt{rand}})$ denotes the probability weights of selecting different types. This procedure is repeated for specified number of times $N_r$ to create a batch $\mathcal{B}$. Finally, for every sample in
$\mathcal{B}$ we add a paraphrased positive $\hat{x_i}^r$ sample thus creating the final batch of size $6N_r$. 

% Next, for every sample in $\mathcal{B}$  add a sample corresponding to a question paraphrase to the $\mathcal{B}_r$. The set $\mathcal{B}_r$ contains the augmented sample corresponding to each sample in $\mathcal{B}$. \\

\textbf{Batch Curation for \lce{}}: We randomly sample batches for cross entropy iterations of size $6N_r$. \\


% To summarize, we use the batches created in Algorithm~\ref{alg:batch} to learn a robust VQA model by alternately training with Cross-Entropy loss(\lce{}) and the SCL loss(\lscl{}) as in Eq~\eqref{loss:vqa}.

% \begin{algorithm}[!t]
% \caption{\label{alg:batch} Batch Curation Strategy for \lsscl{}}
% \begin{algorithmic}
%     \STATE \textbf{input:} batch size $6N_r$; train data $\mathcal{X}$; constants $\bm w$
%     \STATE \textbf{function} CURATE($N_r$, $\mathcal{X}$, $\bm w$)
%         \STATE $~~~~$\textcolor{gray}{\# intialize batches}        
%         \STATE $~~~~$ $\mathcal{B} = \phi, \mathcal{B}_r = \phi$
%         \STATE $~~~~$ \textbf{for all} $i\in \{1, \ldots, N_r\}$ \textbf{do}
%         \STATE $~~~~~~~~$ sample $x_i  \!\sim\! \mathcal{X}$
%         %\STATE $~~~~~~~~$\textcolor{gray}{\# sample intra-class positive}        
%         \STATE $~~~~~~~~$ sample intra-class positive $\hat{x_i}^{p}  \!\sim\! \mathcal{P}(x_i) - \mathcal{P}^r(x_i) $
%         % \STATE $~~~~~~~~$\textcolor{gray}{\# pick negative type}        
%         \STATE $~~~~~~~~$ sample a negative type $t  \!\sim\! D(T \vert \bm w) $
%         \STATE $~~~~~~~~$\textcolor{gray}{\# sample negative from correspoding set}        
%         \STATE $~~~~~~~~$ sample $\bar{x}^{t}_i  \!\sim\!  \mathcal{N}(x_i)^{t}$
%         \STATE $~~~~~~~~$ append $\mathcal{B} = \mathcal{B} \cup \{x_i, \hat{x_i}^{p}, \bar{x}^{t}_i\}$\\

%         \STATE $~~~~$ \textbf{for all} $i\in \{1, \ldots, \vert \mathcal{B} \vert\}$ \textbf{do}
%         %\STATE $~~~~~~~~$\textcolor{gray}{\# sample paraphrased positive}        
%         \STATE $~~~~~~~~$ sample reprphrased positives $\hat{x_i}^{r}  \!\sim\! \mathcal{P}^r(x_i)$
%         \STATE $~~~~~~~~$ append $\mathcal{B}_r = \mathcal{B}_r \{\cup \hat{x_i}^{r}\}$

%     \STATE \textbf{return} $\mathcal{B} \cup \mathcal{B}_r$
% \end{algorithmic}
% \end{algorithm}


\begin{algorithm}[!t]
\caption{\label{alg:batch} Batch Curation Strategy for \lsscl{}}
\begin{algorithmic}
    \STATE \textbf{input:} batch size $6N_r$; train data $\mathcal{X}$; constants $\bm w$
    \STATE \textbf{function} CURATE($N_r$, $\mathcal{X}$, $\bm w$)
        \STATE $~~~~$ $\mathcal{B} = \phi, \mathcal{B}_r = \phi$ \textcolor{gray}{~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\# initialize batches}
        \STATE $~~~~$ \textbf{for all} $i\in \{1, \ldots, N_r\}$ \textbf{do}
        \STATE $~~~~~~~~$$x_i  \!\sim\! \mathcal{X}$ \textcolor{gray}{~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\# reference}
        %\STATE $~~~~~~~~$\textcolor{gray}{\# sample intra-class positive}        
        \STATE $~~~~~~~~$$\hat{x_i}^{p}  \!\sim\! \mathcal{P}(x_i) - \mathcal{P}^r(x_i)$ \textcolor{gray}{~~~~~~~~~~~~~~~~~~\# intra-class positive}
        % \STATE $~~~~~~~~$\textcolor{gray}{\# pick negative type}        
        \STATE $~~~~~~~~$$t  \!\sim\! Cat(T \vert \bm w)$ \textcolor{gray}{~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\# negative type}
        % \STATE $~~~~~~~~$\textcolor{gray}{\# sample negative from correspoding set}        
        \STATE $~~~~~~~~$$\bar{x}^{t}_i  \!\sim\!  \mathcal{N}(x_i)^{t}$ \textcolor{gray}{~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\# negative}
        \STATE $~~~~~~~~$append $\mathcal{B} = \mathcal{B} \cup \{x_i, \hat{x_i}^{p}, \bar{x}^{t}_i\}$\\

        \STATE $~~~~$ \textbf{for all} $i\in \{1, \ldots, \vert \mathcal{B} \vert\}$ \textbf{do}
        %\STATE $~~~~~~~~$\textcolor{gray}{\# sample paraphrased positive}        
        \STATE $~~~~~~~~$$\hat{x_i}^{r}  \!\sim\! \mathcal{P}^r(x_i)$ \textcolor{gray}{~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\# rephrased positive}
        \STATE $~~~~~~~~$append $\mathcal{B}_r = \mathcal{B}_r \{\cup \hat{x_i}^{r}\}$

    \STATE \textbf{return} $\mathcal{B} \cup \mathcal{B}_r$
\end{algorithmic}
\end{algorithm}




==> sections/method_am.tex <==
%% make figure
\begin{figure*}[t!]
  \centering
  \includegraphics[width=\textwidth]{figures/Approachv2.pdf}
  \caption{Dummy caption}
  \label{fig:approach}
\end{figure*}


\section{Preliminaries}
% In this section, we first introduce notations and expand on our VQA architecture that jointly learns V+L representations. 
% Next, we present our modified formulation of Supervised Contrastive Loss \cite{Khosla2020SupervisedCL} 
% for our use case. Finally, expand on the details of our alternate training paradigm and mini-batch creation
% process for the contrastive loss. 
% In this section, we introduce the VQA task and the typical cross entropy training of the VQA models. We then recap contrastive learning and the recently proposed Supervised Contrastive Learning (\SCL/) \cite{Khosla2020SupervisedCL} loss.
In this section, we introduce the VQA task and the typical cross entropy training of the VQA models. We then recap contrastive methods for learning representations~\cite{chen2020simple} and the recently proposed Supervised Contrastive Learning (\SCL/) \cite{Khosla2020SupervisedCL} setup.
%discuss our proposed training paradigm to train VQA models which are robust to minor linguistic variations in the questions. We start with an overview of the VQA dataset and how to augment the dataset with question rephrasings. We then introduce our training paradigm that involves alternately optimizing cross-entropy loss with our variant of the Supervised Contrastive Learning (SCL)~\cite{Khosla2020SupervisedCL} loss. Finally, we describe how carefully curating batches for the two losses can help learn more robust VQA models. 

\textbf{VQA.} 
The Visual Question Answering (VQA)~\cite{vqa,goyal2016making} dataset $\mathcal{D}$ of triplets consisting of an image $v$, a question $q$ and its ground-truth answer $a$ represented as $(v, q, a), \ \forall \ x \in \mathcal{D}$. Given an image-question pair, a VQA model takes as input an image-question pair and produces a distribution over a fixed answer vocabulary. The model takes image and question as input and outputs a joint vision and language (V+L) representation $\bm h \in \mathcal{R}^{d}$ using a multi-modal attention network $f^{mmt}$:
% $$\bm{h} = f^{mmt}(v, q; \theta^{mmt})$$
$$\bm{h} = f^{mmt}(v, q)$$


The V+L representations $\bm{h}$ is used to predict a probability distribution over the answer space $\mathcal{A}$ with a simple softmax classifier $f^{c}(\bm h)$ which is learned via cross-entropy:

\begin{equation}
\begin{aligned}
        \mathcal{L}_{\text{CE}} = -log\frac{\exp(f^c(\bm h)[a])}{\sum_{a'\in \mathcal{A}}\exp(f^c(\bm h)[a'])}
        % \bm h &= f^{mmt}(v,q)\\
        % \mathcal{L}_{ce} = \min_{\theta} &-\mathbb{E_{\mathcal{X}}}[\log p_{\theta}(a|v,q)]
\end{aligned}
\end{equation}
where $f^c(\bm h)[a]$ is the logit corresponding to the answer $a$.

\textbf{Contrastive Learning.} Recent works in vision \cite{chen2020simple} have used contrastive losses to bring representations of two augmented views of the same image (called positives) closer together while pulling apart the representations of two different images (called negatives). %Following recent works in contrastive learning \cite{chen2020simple,Khosla2020SupervisedCL}, we want to bring joint V+L representations obtained from  the question and its paraphrase to be closer together while pulling apart the V+L representations for questions with different answers. 
\yk{Try to rephrase the next statement better} In this, the obtained representation $h = f(x)$ is projected  into a $d$-dimensional hyper-sphere normalized vector $z = g(h) \in \mathcal{R}^{d}$. Next, given a mini-batch of size $K$, the representations are learned by minimizing the InfoNCE~\cite{Oord2018RepresentationLW} loss which operates on representations belonging to pair of positives $(z_i,z_p)$ and $K-1$ negatives $(z_i,z_k), k\in \{1...K\}, k\neq i$ as below:

\begin{equation}
\label{eq:nce_loss}
    \mathcal{L}_{\text{NCE}}^{i} = -\log \frac{\exp(\Phi(\bm z_i, \bm z_p)/\tau)}{\sum_{k=1}^{K} \mathbbm{1}_{k \neq i}\exp(\Phi(\bm z_i, \bm z_k)/\tau)}~,
\end{equation}
where $\mathrm{\Phi}(\bm u,\bm v) = \bm u^\top \bm v / \lVert\bm u\rVert \lVert\bm v\rVert$ computes similarity between $\bm u$ and $\bm v$ and $\tau > 0$ is a scalar temperature parameter.

A generalization of InfoNCE loss to handle more than one positive-pair was proposed by \cite{Khosla2020SupervisedCL} called Supervised Contrastive Loss (SCL). Given a reference sample $x$, SCL uses class-label information to form a set of positives $\mathcal{X}^{+}(x)$. More specifically, $\mathcal{X}^{+}(x)$ contains augmented views of the sample $x$ and samples with same ground truth as $x$. For a minibatch with $K$ samples, \SCL/ is formally defined as:
% The \SCL/ loss given a reference sample $x_i$ and corresponding set of positives denoted by $\mathcal{P}(x_i)$ 
% The set of positives $\mathcal{P}(x_i)$ also contain augmented views of the sample $x_i$ since they also have the same ground-truth label as $x$.
\begin{gather}
%\begin{align}
\mathcal{L}_{\text{SC}}^{i} = -\sum_{p=1}^{\vert \mathcal{X}^{+}(x_i) \vert} { \log \frac{\exp(\Phi(\bm z_i.\bm z_p)/\tau)}{\sum_{k=1}^{K}{\mathbbm{1}_{k \neq i}
\cdot \exp(\Phi(\bm z_i.\bm z_p)/\tau)}}}\nonumber \\
\mathcal{L}_{\text{SC}} = \sum_{i = 1}^{K}{\frac{\mathcal{L}_{\text{SC}}^{i}}{\vert \mathcal{X}^{+}(x_i) \vert}} \label{eq:scl_i}
%\end{align}
 \end{gather}
Overall, \SCL/ tries to bring the representation of samples $x_i$ and $\hat{x}_i \in \mathcal{X}^{+}(x_i)$ closer together compared to representations of samples that have different ground-truth label.

\section{Approach}
We now describe our proposed training paradigm, ConCAT, that uses alternate contrastive and cross-entropy training to learn VQA models robust to question rephrasings. 
 
\textbf{Contrastive Learning in VQA.} For a sample $x = (v, q, a) \ \in \mathcal{D}$, let's denote a set of paraphrases for question $q$ by $\mathcal{Q}(q)$ and the corresponding 
set of VQA triplets: 

$$\mathcal{X}'(x) = \{(v', q', a') \ |\  q' \in \mathcal{Q}(q), v' = v, a' = a \}$$

We also define the set of all samples with the same ground truth answer as $x$ by: 
$$\xpos(x) = \{(\hat{v}, \hat{q}, \hat{a}) \in \mathcal{D} \mid \hat{a} = a \}$$ 

Also, $\xpara(x) \subset \xpos(x)$ as all question rephrasings have the same answer for a given image but not all questions with the same answer are paraphrases of each other. We refer to samples in set $\xpos(x) - \xpara(x)$ as \textit{intra-class} positives and set $\mathcal{X}'{(x)}$ as \textit{paraphrased} positives w.r.t. $x$. \yk{How to simplify next statement} We augment the VQA dataset $\mathcal{D}$ with a set of triplets $\xpara(x)$ formed using multiple paraphrases of a question belonging to all the samples in $\mathcal{D}$. We denote the augmented dataset with $\mathcal{D}^{aug}$. We generate these paraphrases
either by using \BT/~\cite{edunov2018understanding} or a \VQG/ model~\cite{shah2019cycle} .

Ideally, we would like our VQA model to produce the \textit{same and correct} answer for a question and its paraphrase on the same input image. This motivates us to map joint V+L representations of an original and paraphrased sample closer to each other. Moreover, since we operate 
in a supervised setting, following learning~\cite{Khosla2020SupervisedCL} we also try to bring the joint representations for the questions with the same answer (intra-class positives) closer together while pulling apart the representations of questions with different answers. 

Using $\xpos(x_i)$ in Eq\eqref{eq:scl_i} will treat paraphrased question and question with the same answer equally. 
% Similar to using just cross-entropy loss on the augmented dataset, 
SCL loss fails to emphasize the link between question and its paraphrase, to overcome this, we propose a variant of the SCL loss in Eq\eqref{eq:sscl_i} which assigns higher weight to paraphrased positives $\xpara(x)$ over intra-class positives $\xpos(x) - \xpara(x)$. 
Formally, we introduce a scaling factor $\alpha_{ip}$ in the SCL loss (Eq\eqref{eq:scl_i}) for a sample $x_i$ as follows: 
\begin{equation}
\lssc^{i} = -\sum_{p=1}^{\vert \xpos(x_i) \vert} {\alpha_{ip} \cdot \log \frac{\exp(\Phi(\bm z_i.\bm z_p)/\tau)}{\sum_{k=1}^{N}{\mathbbm{1}_{k \neq i}
\cdot \exp(\Phi(\bm z_i.\bm z_p)/\tau)}}} \label{eq:sscl_i}
\end{equation}
\begin{equation}
% \mathcal{L}_{sscl} = \sum_{i = 1}^{K}{\frac{\mathcal{L}^{i}_{scl}}{\sum_{p=1}^{\vert \mathcal{P}(x_i) \vert}\alpha_{ip}}} 
\lssc = \sum_{i = 1}^{K}{\frac{\lssc^{i}}{\sum_{p}\alpha_{ip}}} 
\end{equation}

The scaling factor $\alpha_{ip}$ assigns a higher weight $\alpha>1$ to positive samples corresponding to question paraphrases compared to other intra-class positives. Intuitively, because of the higher weight, the loss will penalize the model strongly if it fails to bring 
the representations of a question and its paraphrase closer. Formally, we define $\alpha_{ip}$ as: 
\begin{equation}
\label{eq:alpha}
\alpha_{ip} = 
\begin{cases}
    \alpha& \text{if } x_p \in \mathcal{X'}(x_i),   \\
    1,              & \text{otherwise}
\end{cases}
\end{equation}

\subsection{Alternate Training} \label{ssec:alt}
In contrast with \cite{Khosla2020SupervisedCL} who pretrain their network using \lscl{} and finetune it on cross-entropy \lce{}, we train our model by alternating between \lsscl{}  and the cross-entropy \lce{}  iterations. The benefit of our approach is twofold: First, training alternately allows us to curate batches with multiple-positives and hard-negatives (see \ref{ssec:batchmining}{next section}) for \lsscl{} without affecting the \lce{}. Second, we have a single-stage training compared to two-stage training in \cite{Khosla2020SupervisedCL} which usually doubles the hyper-parameter tuning efforts and training iterations. 
% The benefit of our approach is twofold: The main advantage of alternate training compared to two-stage training in \cite{Khosla2020SupervisedCL} is that it allows us to curate loss-specific batches with multiple-positives and hard-negatives (see \ref{ssec:batchmining} for \lscl{} that further boosts the performance without affecting the \lce{}.  
Our training paradigm is summarized in Algorithm \ref{alg:main}. Specifically, given $N$ total training iterations, we update our model with \lscl{} after every $N_{ce}-1$ updates with \lce{}, where $N_{ce}$ is a hyper-parameter. Our overall loss for the $n^{th}$ iteration $\forall n \in [1,N]$ can be written as: 
\begin{equation}
    \label{loss:vqa}
    \mathcal{L}_n = \mathbbm{1}_{n\Mod{N_{ce}} = 0} \cdot \lssc + \mathbbm{1}_{n\Mod{N_{ce}} \neq 0} \cdot \mathcal{L}_{\text{CE}}
\end{equation}
% \am{mention $\forall n \in {1,...,N}$ somewhere.}


\begin{algorithm}[t]
\caption{\label{alg:main} \concat/ with \lsscl{} and \lce{}}
\begin{algorithmic}
    \STATE \textbf{input:} steps $N$; constant $N_{ce}$; train data $\mathcal{D}$; networks $f,g$
    % \STATE \textbf{function} CURATE($N_r$, $\mathcal{X}$, $\tau$, $\bm \alpha$)
        % \STATE $~~~~$\textcolor{gray}{\# intialize batches}        
        % \STATE $~~~~$ $\mathcal{B} = \phi, \mathcal{B}_r = \phi$
        \STATE $~~~~$ \textbf{for all} $i\in \{1, \ldots, N\}$ \textbf{do}
        \STATE $~~~~~~~~$ $\mathcal{B} = \phi$

        \STATE $~~~~~~~~$ \textbf{if} $i \Mod{N_{ce}} = 0$ \textbf{do}
        \STATE $~~~~~~~~~~~$\textcolor{gray}{\# scl iteration}        
        \STATE $~~~~~~~~~~~$$\mathcal{B}=$ CURATE($N_r$, $\mathcal{D}$, $\bm w$); $\mathcal{L}=$ \lscl{}
        % \STATE $~~~~~~~~$ $\mathcal{L}= \mathcal{L}_{scl}$

        \STATE $~~~~~~~~$ \textbf{else} \textbf{do}
        \STATE $~~~~~~~~~~~$\textcolor{gray}{\# ce iteration}
        \STATE $~~~~~~~~~~~$$\mathcal{B} \!\sim\! \mathcal{D}$; $\mathcal{L}=$ \lce{}
        \STATE $~~~~~~~~$ update $f(.),g(.)$ networks to minimize $\mathcal{L}$ over $\mathcal{B}$
        
    \STATE \textbf{return} network $f(.)$; throw away $g(.)$
\end{algorithmic}
\end{algorithm}

\subsection{Negative Types and Batch Creation} \label{ssec:batchmining}
Any contrastive loss including SCL operates with multiple negative samples. 
% We define a set of negatives $\mathcal{N}(x) \subseteq \mathcal{X}^{aug}$ for any reference sample $x \in \mathcal{X}^{aug}$ as a collection of samples that have a different answer than the sample:
For a given reference sample $x = (v, q, a) \in \mathcal{D}^{aug}$, we define a corresponding set of negatives as samples with ground truth different than the reference $x$:
\begin{equation*}
    \xneg(x) = \{ (\bar{v}, \bar{q}, \bar{a})\in \mathcal{D}^{aug} \mid  \bar{a}\neq a \}
\end{equation*}


% The minibatches for \lscl{} in~\cite{Khosla2020SupervisedCL} are created by first sampling a set of anchor samples and the corresponding positive pairs. For every sample, other samples in the minibatch with a different ground-truth label is considered negative. 

We carefully curate batches for \lsscl{} by sampling different types of negatives. Given $\bar{x} = (\bar{v}, \bar{q}, \bar{a} ) \in \xneg(x)$, we classify a negative pair $({x}, \bar{x})$ into one of three negative categories from $\mathcal{T}=$ \texttt{[que, img, rand]} via a mapping function $\Omega:{\mathcal{D} \times \mathcal{D}} \rightarrow \mathcal{T}$ such that:
\begin{equation}
\Omega({x}, \bar{x}) = 
\begin{cases}
    \texttt{img}  & \text{if } v = \bar{v}  \\
    \texttt{que}  & \text{if } sim(q, \bar{q}) > \epsilon  \\
    \texttt{rand} &  \text{else}
\end{cases}
\end{equation}

where $\epsilon$ is a similarity threshold. We use $\epsilon=0.95$ for our experiments. We now partition $\xneg(x)$ in three mutually exclusive subsets $\xneg_t(x), t \in \mathcal{T}$ defined as:
\begin{equation}
    \xneg_t(x) = \{\bar{x} \in \xneg(x) \mid \Omega({x}, \bar{x}) = t \}
\end{equation} 

\begin{itemize}
    \item \textbf{Image Negatives}, ($ \xneg_{\texttt{img}}(x)$): Image negatives are samples 
    that have same image as the reference ($x$) but different answer. Since VQA dataset has multiple questions ($\sim$ 5.4) per image, finding image negatives is trivial. 
    \item \textbf{Question Negatives}, ($ \xneg_{\texttt{que}}(x)$):  Question negatives are samples with similiar questions and different answers. We measure the similarity between the questions by computing their cosine distance in the vector space of the Sentence-BERT \cite{reimers2019sentencebert} model.
    % The similarity between the questions is computed by using representations from Sentence-BERT introduced by \cite{reimers2019sentencebert}.
    \item \textbf{Random Negatives}, ($ \xneg_{\texttt{rand}}(x)$): Random negatives are samples do not fall under either Image or Question negative categories.
\end{itemize}

We hypothesize that discriminating between joint V+L representations of above negatives and the reference would lead to more robust V+L representations as it requires the model to preserve relevant information of both modalities in the learnt representation. Negative samples belonging to each of the above types are depicted in Figure \ref{fig:approach}. \\

\textbf{Batch Curation}: To create mini-batches for \lsscl/, as described in Algorithm~\ref{alg:batch}, we start by filling our batch with triplets of reference $x_i$, a intra-class positive $\hat{x_i}$ and a negative sample $\bar{x_i}$ of type $t$. The negative type $t$ is sampled from a categorical distribution $\text{Cat}(\mathcal{T} \vert\bm w)$ where $\bm w = (w_{\texttt{img}}, w_{\texttt{que}}, w_{\texttt{rand}})$ are the probability weights of selecting different types. This procedure is repeated for specified number of times $N_r$ to create a batch $\mathcal{B}$. Finally, for every sample in $\mathcal{B}$ we add a corresponding paraphrased positive ${x'_i}$ sample. For \lce{}, we randomly add samples from the training dataset $\mathcal{D}$ to the mini-batch. 
% Next, for every sample in $\mathcal{B}$  add a sample corresponding to a question paraphrase to the $\mathcal{B}_r$. The set $\mathcal{B}_r$ contains the augmented sample corresponding to each sample in $\mathcal{B}$. \\
% To summarize, we use the batches created in Algorithm~\ref{alg:batch} to learn a robust VQA model by alternately training with Cross-Entropy loss(\lce{}) and the SCL loss(\lscl{}) as in Eq~\eqref{loss:vqa}.

% \begin{algorithm}[!t]
% \caption{\label{alg:batch} Batch Curation Strategy for \lsscl{}}
% \begin{algorithmic}
%     \STATE \textbf{input:} batch size $6N_r$; train data $\mathcal{X}$; constants $\bm w$
%     \STATE \textbf{function} CURATE($N_r$, $\mathcal{X}$, $\bm w$)
%         \STATE $~~~~$\textcolor{gray}{\# intialize batches}        
%         \STATE $~~~~$ $\mathcal{B} = \phi, \mathcal{B}_r = \phi$
%         \STATE $~~~~$ \textbf{for all} $i\in \{1, \ldots, N_r\}$ \textbf{do}
%         \STATE $~~~~~~~~$ sample $x_i  \!\sim\! \mathcal{X}$
%         %\STATE $~~~~~~~~$\textcolor{gray}{\# sample intra-class positive}        
%         \STATE $~~~~~~~~$ sample intra-class positive $\hat{x_i}^{p}  \!\sim\! \mathcal{P}(x_i) - \mathcal{P}^r(x_i) $
%         % \STATE $~~~~~~~~$\textcolor{gray}{\# pick negative type}        
%         \STATE $~~~~~~~~$ sample a negative type $t  \!\sim\! D(T \vert \bm w) $
%         \STATE $~~~~~~~~$\textcolor{gray}{\# sample negative from correspoding set}        
%         \STATE $~~~~~~~~$ sample $\bar{x}^{t}_i  \!\sim\!  \mathcal{N}(x_i)^{t}$
%         \STATE $~~~~~~~~$ append $\mathcal{B} = \mathcal{B} \cup \{x_i, \hat{x_i}^{p}, \bar{x}^{t}_i\}$\\

%         \STATE $~~~~$ \textbf{for all} $i\in \{1, \ldots, \vert \mathcal{B} \vert\}$ \textbf{do}
%         %\STATE $~~~~~~~~$\textcolor{gray}{\# sample paraphrased positive}        
%         \STATE $~~~~~~~~$ sample reprphrased positives $\hat{x_i}^{r}  \!\sim\! \mathcal{P}^r(x_i)$
%         \STATE $~~~~~~~~$ append $\mathcal{B}_r = \mathcal{B}_r \{\cup \hat{x_i}^{r}\}$

%     \STATE \textbf{return} $\mathcal{B} \cup \mathcal{B}_r$
% \end{algorithmic}
% \end{algorithm}


\begin{algorithm}[!t]
\caption{\label{alg:batch} Batch Curation Strategy for \lsscl{}}
\begin{algorithmic}
    \STATE \textbf{input}: number of references $N_r$; train data $\mathcal{D}$; weights $\bm w$
    \STATE \textbf{function} CURATE($N_r$, $\mathcal{D}$, $\bm w$)
        \STATE $~~~~$ $\mathcal{B} = \phi, \mathcal{B}_r = \phi$ \textcolor{gray}{~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\# initialize batches}
        \STATE $~~~~$ \textbf{for all} $i\in \{1, \ldots, N_r\}$ \textbf{do}
        \STATE $~~~~~~~~$$x_i  \!\sim\! \mathcal{D}$ \textcolor{gray}{~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\# reference}
        %\STATE $~~~~~~~~$\textcolor{gray}{\# sample intra-class positive}        
        \STATE $~~~~~~~~$$\hat{x_i}  \!\sim\! \xpos(x_i) - \xpara(x_i)$ \textcolor{gray}{~~~~~~~~~~~~~\# intra-class positive}
        % \STATE $~~~~~~~~$\textcolor{gray}{\# pick negative type}        
        \STATE $~~~~~~~~$$t  \!\sim\! \text{Cat}(\mathcal{T} \vert \bm w)$ \textcolor{gray}{~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\# negative type}
        % \STATE $~~~~~~~~$\textcolor{gray}{\# sample negative from correspoding set}        
        \STATE $~~~~~~~~$$\bar{x}_i  \!\sim\!  \xneg_{t}(x_i)$ \textcolor{gray}{~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\# negative}
        \STATE $~~~~~~~~$append $\mathcal{B} = \mathcal{B} \cup \{x_i, \hat{x_i}, \bar{x}_i\}$\\

        \STATE $~~~~$ \textbf{for all} $i\in \{1, \ldots, \vert \mathcal{B} \vert\}$ \textbf{do}
        %\STATE $~~~~~~~~$\textcolor{gray}{\# sample paraphrased positive}        
        \STATE $~~~~~~~~$${x'_i}  \!\sim\! 
        \xpara(x_i)$ \textcolor{gray}{~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\# paraphrased positive}
        \STATE $~~~~~~~~$append $\mathcal{B}_r = \mathcal{B}_r \cup \{x'_i\}$
    \STATE \textbf{return} $\mathcal{B} \cup \mathcal{B}_r$
\end{algorithmic}
\end{algorithm}




==> sections/scratch-table.tex <==
\newcommand{\band}{\rowcolor{gray!10}}
\begin{table*}[t!]\footnotesize
\setlength\tabcolsep{3.5pt}
\renewcommand{\arraystretch}{1.25}
\center
\caption{Results on TextVQA \cite{Singh2019TowardsVM} dataset. We compare our model (rows 11-13) against the prior works (row 1-5) and the improved baselines (rows 6-10).
% \cite{Singh2019TowardsVM, textvqa_dcd, textvqa_msft_vti, hu2019iterative}. 
% Structure denotes the model composition, e.g. 2N\rarrow4S model contains 2 normal and 4 \spat \ transformer layers.
\\ \scriptsize{$^{\dagger}$ Indicates our ablations for improved baseline.\\$^{\dagger \dagger}$ Indicates the best model from improved baseline.}}
\resizebox{0.73\textwidth}{!}{
\begin{tabular}{llccccccc}
\toprule
& Method & Structure & \makecell{OCR \\ system} & \makecell{DET \\backbone} & \makecell{w/ \\ ST-VQA} & \makecell{Beam \\ size} & \makecell{Accu. \\ on val} & \makecell{Accu. \\ on test} \\
\midrule
\band \small\texttt{1} & LoRRA \cite{Singh2019TowardsVM} & - & R-ml & ResNet & \xmark & - & 26.5 & 27.6\\
\small\texttt{2} & DCD \cite{textvqa_RTArt} & - & - & - & - & - & 31.4 & 31.4\\
\band \small\texttt{3} & MSFT \cite{textvqa_msft_vti} & - & - & - & - & - & 32.9 & 32.4\\
\small\texttt{4} & M4C \cite{hu2019iterative} & 4N & R-en & ResNet &  \xmark & 1 & 39.4 & 39.0 \\
\band \small\texttt{5} & M4C \cite{hu2019iterative} & 4N & R-en & ResNet &  \cmark & 1 & 40.5 & 40.4\\
\midrule
\small\texttt{6} & M4C \cite{hu2019iterative}$^{\dagger}$ & 4N & G & ResNet & \xmark & 1 & 41.8 & - \\
\band \small\texttt{7} & M4C \cite{hu2019iterative}$^{\dagger}$ & 4N & G & ResNeXt & \xmark& 1 & 42.0 & - \\
\small\texttt{8} & M4C \cite{hu2019iterative}$^{\dagger}$ & 6N & G & ResNeXt & \xmark& 1 & 42.7 & - \\
\band \small\texttt{9} &  M4C \cite{hu2019iterative}$^{\dagger}$ & 6N & G & ResNeXt & \cmark & 1 & 43.3 & - \\
\small\texttt{10} &  M4C \cite{hu2019iterative}$^{\dagger \dagger}$ & 6N & G & ResNeXt & \cmark & 5 & 43.8 & 42.4\\
\midrule
\band \small\texttt{11} & \SAM \ (ours) & 2N\rarrow4S & G & ResNeXt & \xmark & 1 & 43.9 & -\\
\small\texttt{12} & \SAM \ (ours) & 2N\rarrow4S & G & ResNeXt & \cmark & 1 & 45.1 & - \\
\band \small\texttt{13} & \SAM \ (ours) & 2N\rarrow4S & G & ResNeXt & \cmark & 5 & \textbf{45.4} & \textbf{44.6} \\
\bottomrule
\end{tabular}}
\smallskip
\label{tab:textvqa}
\vspace{-15pt}
\end{table*}
\clearpage




%
% 
% 

\begin{table}[t]\centering
\setlength{\tabcolsep}{3.5pt}
\begin{tabular}{lcccccccccccc}
 \toprule
  \multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{Loss}} & \multirow{2}{*}{\textbf{DA}} & \multirow{2}{*}{\textbf{Scaling}} & \multicolumn{4}{c}{\textbf{Consensus Score(k)}} & \multicolumn{5}{c}{\textbf{VQA Accuracy}} \\
%   \cmidrule(l{0.6em}r{0.65em}){5-8} \cmidrule(l{0.55em}r{0.6em}){9-13}
  ~ & ~ & ~ & ~ & \textbf{k=1} & \textbf{k=2} & \textbf{k=3} & \textbf{k=4} & \textbf{ORI} & \textbf{REP} & \textbf{val} & \textbf{test-dev}& \textbf{test-std} \\
 \midrule
 Pythia~\cite{pythia18arxiv} & & &    & 63.43	& 52.03	& 45.94	& 39.49	& 64.08	& 54.20 \\
 Pythia + CC                 & & &  & \textbf{64.36}	& \textbf{55.45}	& \textbf{50.92}	& \textbf{44.30}	& \textbf{64.52}	& \textbf{55.65}\\
 \midrule
 BAN~\cite{Kim2018}          & &  &   & 64.88	& 53.08	& 47.45	& 39.87	& 64.97	& 55.87 \\
 BAN + CC                    & &  &  & \textbf{65.77}	& \textbf{56.94}	& \textbf{51.76}	& \textbf{48.18}	& \textbf{65.87}	& \textbf{56.59} \\ 
\midrule
UNITER & CE & None & \xmark & -1 & -1 & -1 & -1 & -1 & -1 & -1 & -1 & -1  \\
UNITER & CE & BT & \xmark & -1 & -1 & -1 & -1 & -1 & -1 & -1 & -1 & -1 \\
UNITER & CE + SCL (J) & BT & \xmark & -1 & -1 & -1 & -1 & -1 & -1 & -1 & -1 & -1 \\
UNITER & CE + SCL (A) & BT & \xmark & -1 & -1 & -1 & -1 & -1 & -1 & -1 & -1 & -1 \\
\end{tabular}
  \caption{\textbf{Consensus performance on \vqarep dataset}. CS(k) as defined in Eq.~\ref{eq:consesus_score} is consensus score which is non-zero only if \emph{at least} $k$ rephrasings are answered correctly, zero otherwise; averaged across all group of questions.
  %
  ORI represent a split of questions from \vqarep which are original questions from VQA v2.0 and their corresponding rephrasings are represented by the split REP.
  %
  Models trained with our cycle-consistent (CC) framework consistently outperform their baseline counterparts at all values of $k$.
  }
  \label{robustness_table}
\end{table}
\clearpage
% 
% 
% 
% 

usepackage{booktabs}
\newcommand{\ra}[1]{\renewcommand{\arraystretch}{#1}}

\begin{table*}\centering
\ra{1.3}
\begin{tabular}{@{}rrrrcrrrcrrr@{}}\toprule
& \multicolumn{3}{c}{$w = 8$} & \phantom{abc}& \multicolumn{3}{c}{$w = 16$} &
  \phantom{abc} & \multicolumn{3}{c}{$w = 32$}\\
\cmidrule{2-4} \cmidrule{6-8} \cmidrule{10-12}
  & $t=0$ & $t=1$ & $t=2$ && $t=0$ & $t=1$ & $t=2$ && $t=0$ & $t=1$ & $t=2$\\\midrule
$dir=1$\\
$c$ & 0.0790 & 0.1692 & 0.2945 && 0.3670 & 0.7187 & 3.1815 && -1.0032 & -1.7104 & -21.7969\\
$c$ &  -0.8651& 50.0476& 5.9384&& -9.0714& 297.0923& 46.2143&& 4.3590& 34.5809& 76.9167\\
$c$ & 124.2756& -50.9612& -14.2721&& 128.2265& -630.5455& -381.0930&& -121.0518& -137.1210& -220.2500\\

$dir=0$\\
$c$ & 0.0357& 1.2473& 0.2119&& 0.3593& -0.2755& 2.1764&& -1.2998& -3.8202& -1.2784\\
$c$ & -17.9048& -37.1111& 8.8591&& -30.7381& -9.5952& -3.0000&& -11.1631& -5.7108& -15.6728\\
$c$ & 105.5518& 232.1160& -94.7351&& 100.2497& 141.2778& -259.7326&& 52.5745& 10.1098& -140.2130\\

\bottomrule
\end{tabular}
\caption{Caption}
\end{table*}


%##################################################################################################
\begin{algorithm}[t]
\caption{Pseudocode of batch creation for SCL}
\label{alg:code}
\algcomment{\fontsize{7.2pt}{0em}\selectfont \texttt{bmm}: batch matrix multiplication; \texttt{mm}: matrix multiplication; \texttt{cat}: concatenation.
%\vspace{-1.em}
}
\definecolor{codeblue}{rgb}{0.25,0.5,0.5}
\lstset{
  backgroundcolor=\color{white},
  basicstyle=\fontsize{7.2pt}{7.2pt}\ttfamily\selectfont,
  columns=fullflexible,
  breaklines=true,
  captionpos=b,
  commentstyle=\fontsize{7.2pt}{7.2pt}\color{codeblue},
  keywordstyle=\fontsize{7.2pt}{7.2pt},
%  frame=tb,
}
\begin{lstlisting}[language=python]

def get_scl_batch():
    
    # initialize batch
    batch = []
    for x in loader:
        # get sample with same groud-truth as x
        x_pos = get_same_gt(loader, x)
        
        # add both x, x_pos to the batch
        batch.extend([x, x_pos])
        
        # finish when you have enough samples
        len(batch) == num_ref:
            break
    
    # fill with negatives
    while True:
        # cycle over samples in the batch
        x = next_sample(batch) 
        
        # pick type from ["question", "image", "random"]
        neg_type = weighted_sampling(types, weights)
        
        # get the negative sample
        x_neg = get_negative(loader, neg_type, x)
        
        # add x_neg to batch
        batch.extend([x_neg])
        
        # finish when batch is complete
        if len(batch) == batch_size:
            break
    
    # generate data-augmented batch
    da_batch = []
    for x in batch:
        
        # get a rephrased sample corresponding to x
        x_aug = get_da(loader, x)
        
        # add x_aug to da_batch
        da_batch.extend([x_aug])
    
    # return both the batches
    return batch, da_batch

\end{lstlisting}
\end{algorithm}
%##################################################################################################

\begin{algorithm}[!t]
\caption{\label{alg:main} SimCLR's main learning algorithm.}
\begin{algorithmic}
    \STATE \textbf{input:} batch size $N$, constant $\tau$, structure of $f$, $g$, $\mathcal{T}$.
\FOR{sampled minibatch $\{\bm x_k\}_{k=1}^N$}
    \STATE \textbf{for all} $k\in \{1, \ldots, N\}$ \textbf{do}
        \STATE $~~~~$draw two augmentation functions $t \!\sim\! \mathcal{T}$, $t' \!\sim\! \mathcal{T}$
        \STATE $~~~~$\textcolor{gray}{\# the first augmentation} \STATE $~~~~$$\tilde{\bm x}_{2k-1} = t(\bm x_k)$
        \STATE $~~~~$$\bm h_{2k-1} = f(\tilde{\bm x}_{2k-1})$  \textcolor{gray}{~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\# representation}
        \STATE $~~~~$$\bm z_{2k-1} = g({\bm h}_{2k-1})$  \textcolor{gray}{~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\# projection}
        \STATE $~~~~$\textcolor{gray}{\# the second augmentation} \STATE $~~~~$$\tilde{\bm x}_{2k} = t'(\bm x_k)$
        \STATE $~~~~$$\bm h_{2k} = f(\tilde{\bm x}_{2k})$      \textcolor{gray}{~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\# representation}
        \STATE $~~~~$$\bm z_{2k} = g({\bm h}_{2k})$      \textcolor{gray}{~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\# projection}
    \STATE \textbf{end for}
    \STATE \textbf{for all} $i\in\{1, \ldots, 2N\}$ and $j\in\{1, \dots, 2N\}$ \textbf{do}
    \STATE $~~~~$ $s_{i,j} = \bm z_i^\top \bm z_j / (\lVert\bm z_i\rVert \lVert\bm z_j\rVert)$ \textcolor{gray}{~~~~~~~~\# pairwise similarity}\\
    \STATE \textbf{end for}
    \STATE \textbf{define} $\ell(i, j)$ \textbf{as}~ $\ell(i, j) \!=\! -\log \frac{\exp(s_{i,j}/\tau)}{\sum_{k=1}^{2N} \one{k \neq i}\exp(s_{i, k}/\tau)}$ \\ \STATE $\mathcal{L} = \frac{1}{2N} \sum_{k=1}^N \left[ \ell(2k\!-\!1, 2k) + \ell(2k, 2k\!-\!1)\right]$
    \STATE update networks $f$ and $g$ to minimize $\mathcal{L}$
    \ENDFOR
    \STATE \textbf{return} encoder network $f(\cdot)$, and throw away $g(\cdot)$
\end{algorithmic}
\end{algorithm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table*}[h!]\centering
\setlength{\tabcolsep}{3.5pt}
\begin{tabular}{clccccccccccccc}
 \toprule
  \multirow{2}{*}{} & \multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{DA}} & \multirow{2}{*}{\textbf{Scale}}& \multirow{2}{*}{\textbf{N-Type}} & \multicolumn{4}{c}{\textbf{Consensus Score(k)}} & \multicolumn{3}{c}{\textbf{VQA Accuracy}} \\

%   \multirow{2}{*}{} & \multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{Loss}} & \multirow{2}{*}{\textbf{DA}} & \multirow{2}{*}{\textbf{Scale}}& \multirow{2}{*}{\textbf{N-Type}} & \multicolumn{4}{c}{\textbf{Consensus Score(k)}} & \multicolumn{3}{c}{\textbf{VQA Accuracy}} \\

%   \cmidrule(l{0.6em}r{0.65em}){5-8} \cmidrule(l{0.55em}r{0.6em}){9-13}
  ~ &  ~ &  ~ & ~ & ~ & \textbf{k=1} & \textbf{k=2} & \textbf{k=3} & \textbf{k=4} & \textbf{val} & \textbf{test-dev}&  \textbf{test-dev \texttt{[train]}} \\
 \midrule
 \band  \small\texttt{1} & Pythia~\shortcite{jiang2018pythia}  &- &- &  - & 63.43	& 52.03	& 45.94	& 39.49	&65.78	& - & -  \\
 \small\texttt{2} &  BAN~\shortcite{kim2018bilinear}          & - &- & - & 64.88	& 53.08	& 47.45	& 39.87	& 66.04	& - & - \\
\band  \small\texttt{3} &  Pythia + CC~\shortcite{shah2019cycle}               &- & -&- & {64.36}	& {55.45}	& {50.92}	& {44.30}	& {66.03}	& {-} & -\\
\small\texttt{4} &  BAN + CC~\shortcite{shah2019cycle}                    & - &- & -& {65.77}	& {56.94}	& {51.76}	& {48.18}	& {66.77}	& {-} & - \\ 
\midrule
\band  \small\texttt{5} & MMT + CE   & - &  - & - & 67.74 & 59.82 & 55.10 & 51.82 & 66.46 & 68.05 & -   \\
\midrule
 \small\texttt{6} & MMT + CE  & VQG & - & - & 66.53 & 59.26 & 54.92 & 51.85 & 64.50 &  66.08 & - \\
\band  \small\texttt{7} & MMT + ConCAT   & VQG & \ding{51} & \texttt{RQI} & 66.49 & 59.55 & 55.33 & 52.31 & 64.74 & 66.30 & -\\
\midrule
 \small\texttt{8} & MMT + CE   & BT & - & - & 67.58 & 60.04 & 55.53 & 52.36 & 66.31 & 67.85 & - \\
% \band  \small\texttt{7} & MMT  & CE + SCL (J-R) & BT & \xmark & \texttt{R} & 67.22 & 59.92 & 55.54 & 52.43 & 65.57 & 67.13 & -1 \\
%  \small\texttt{7} & MMT  &  + SCL (J-S) & BT & \xmark & \texttt{R} & 66.95 & 59.70 & 55.32 & 52.20 & 65.10 & 66.73 & -1 \\
\band  \small\texttt{9} & MMT + (SCL$\rightarrow$CE) & BT & \xmark & \texttt{R} & 65.34 & 57.39 & 52.63 & 49.20 & 64.21 & 65.83 & -\\
\small\texttt{10} & MMT + (CE + SCL)   & BT & \xmark & \texttt{R} & 66.95 & 59.70 & 55.32 & 52.20 & 65.10 & 66.73 & - \\
\band  \small\texttt{11} & MMT + ConCAT   & BT & \xmark & \texttt{R} & 68.35 & 60.97 & 56.49 & 53.30 & 66.73 & 68.40 & -\\
  \small\texttt{12} & MMT + ConCAT   & BT & \ding{51} & \texttt{R} & 68.19 & 60.92 & 56.53 & 53.42 & 66.62 & 68.26 & -\\
\band \small\texttt{13} & MMT + ConCAT  & BT & \ding{51} & \texttt{RQ} & 68.41 & 61.24 & 56.88 & 53.77 & 66.97 & 68.68 & -\\
 \small\texttt{14} &  MMT + ConCAT   & BT & \ding{51} & \texttt{RI} & 68.47 & 61.28 & 56.91 & 53.79 & 66.93 & 68.60 & -\\
\band \small\texttt{15} & MMT + ConCAT   & BT & \xmark & \texttt{RQI} & 68.20 & 60.90 & 56.49 & 53.36 & 66.60 & 68.21 & -\\
  \small\texttt{16} & MMT + ConCAT   & BT & \ding{51} & \texttt{RQI} & 68.62 & 61.42 & 57.08 & 53.99 & 66.98 & 68.58 & 68.76\\
% \midrule
%  \small\texttt{15} & MMT + (SCL $\rightarrow$ CE) [L]  & BT & \xmark & \texttt{RQI}& 28.36 & 28.36 & 28.36 & 28.36 & 24.04 & 25.70 & - \\
\bottomrule

\end{tabular}
  \caption{\textbf{Ablations on VQA-Rephrasings and VQA 2.0 dataset}. CS(k) as defined in Eq.~\ref{eq:consesus_score} is consensus score which is non-zero only if \emph{at least} $k$ rephrasings are answered correctly, zero otherwise. \textbf{DA} denotes the source of augemented data from either Back Translation (BT) or Visual Question Generation (VQG). \textbf{N-Type}  defines the type of negatives used from Image (\texttt{I}), Question (\texttt{Q}) and Random (\texttt{R}) as defined in Section \ref{ssec:batchmining}{2}. \textbf{Scale} denotes whether scaling factor $\alpha$ (defined in Eq.~\ref{eq:alpha}) was used.}
  \label{robustness_table}
\end{table*}



==> sections/scratch.tex <==
\ha{Recent Visual Question Answering (VQA) models have shown impressive performance on the VQA benchmark but are very brittle to small linguistic variations in input questions. Existing approaches have tried to address this problem by augmenting the dataset with question paraphrases generated using techniques such as visual question generation models and adversarial perturbations. These approaches fail to fully exploit the augmented data as they use the augmented data to simply learn an answer classifier by minimizing the standard cross-entropy loss. 
Building on top of recent success in contrastive learning, we propose a novel training paradigm that alternately optimize cross-entropy and contrastive losses to better utilize the augmented data. Contrastive loss learns joint vision and language representations which are robust to linguistic variations in questions while cross-entropy loss preserves discriminative power of the representations for answer classification. We show that VQA models trained under our proposed training paradigm achieve higher consistency scores across rephrasings in the VQA-Rephrasings dataset. Additionally, these models also achieve higher VQA accuracy on the VQA 2.0 dataset.}

==> tables/robustness_table.tex <==
\begin{table*}[h!]\centering
\setlength{\tabcolsep}{3.5pt}
\begin{tabular}{clccccccccccccc}
 \toprule
  \multirow{2}{*}{} & \multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{DA}} & \multirow{2}{*}{\textbf{Scaling}}& \multirow{2}{*}{\textbf{N-Type}} & \multicolumn{4}{c}{\textbf{Consensus Score(k)}} & \multicolumn{3}{c}{\textbf{VQA Score}} \\

%   \multirow{2}{*}{} & \multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{Loss}} & \multirow{2}{*}{\textbf{DA}} & \multirow{2}{*}{\textbf{Scale}}& \multirow{2}{*}{\textbf{N-Type}} & \multicolumn{4}{c}{\textbf{Consensus Score(k)}} & \multicolumn{3}{c}{\textbf{VQA Accuracy}} \\

%   \cmidrule(l{0.6em}r{0.65em}){5-8} \cmidrule(l{0.55em}r{0.6em}){9-13}
  ~ &  ~ &  ~ & ~ & ~ & \textbf{k=1} & \textbf{k=2} & \textbf{k=3} & \textbf{k=4} & \textbf{val} & \textbf{test-dev}&  \textbf{test-std} \\
 \midrule
 \band  \small\texttt{1} & Pythia~\cite{jiang2018pythia}  &- &- &  - & 63.43	& 52.03	& 45.94	& 39.49	&65.78	& 68.43 & -  \\
 \small\texttt{2} &  BAN~\cite{kim2018bilinear}          & - &- & - & 64.88	& 53.08	& 47.45	& 39.87	& 66.04	& 69.64 & - \\
\band  \small\texttt{3} &  Pythia + CC~\cite{shah2019cycle}               &- & -&- & {64.36}	& {55.45}	& {50.92}	& {44.30}	& {66.03}	& 68.88 & -\\
\small\texttt{4} &  BAN + CC~\cite{shah2019cycle}                    & - &- & -& {65.77}	& {56.94}	& {51.76}	& {48.18}	& {66.77}	& \textbf{69.87} & - \\ 
\midrule
\band  \small\texttt{5} & MMT + CE   & - &  - & - & 67.74 & 59.82 & 55.10 & 51.82 & 66.46 & - & -   \\
\midrule
 \small\texttt{6} & MMT + CE  & VQG & - & - & 66.53 & 59.26 & 54.92 & 51.85 & 64.50 &  - & - \\
\band  \small\texttt{7} & MMT + ConCAT   & VQG & \ding{51} & \texttt{RQI} & 66.49 & 59.55 & 55.33 & 52.31 & 64.74 & - & -\\
\midrule
 \small\texttt{8} & MMT + CE   & BT & - & - & 67.58 & 60.04 & 55.53 & 52.36 & 66.31 & 69.51 & 69.22 \\
\band  \small\texttt{9} & MMT + (SCL$\rightarrow$CE) & BT & \xmark & \texttt{R} & 65.34 & 57.39 & 52.63 & 49.20 & 64.21 & - & -\\
\small\texttt{10} & MMT + (CE + SCL)   & BT & \xmark & \texttt{R} & 66.95 & 59.70 & 55.32 & 52.20 & 65.10 & - & - \\
% \band  \small\texttt{11} & MMT + ConCAT   & BT & \xmark & \texttt{R} & 68.35 & 60.97 & 56.49 & 53.30 & 66.73 & - & -\\
  \small\texttt{12} & MMT + ConCAT   & BT & \ding{51} & \texttt{R} & 68.19 & 60.92 & 56.53 & 53.42 & 66.62 & - & -\\
\band \small\texttt{13} & MMT + ConCAT  & BT & \ding{51} & \texttt{RQ} & 68.41 & 61.24 & 56.88 & 53.77 & 66.97 & - & -\\
 \small\texttt{14} &  MMT + ConCAT   & BT & \ding{51} & \texttt{RI} & 68.47 & 61.28 & 56.91 & 53.79 & 66.93 & - & -\\
\band \small\texttt{15} & MMT + ConCAT   & BT & \xmark & \texttt{RQI} & 68.20 & 60.90 & 56.49 & 53.36 & 66.60 & - & -\\
\small\texttt{16} & MMT + ConCAT   & BT & \ding{51} & \texttt{QI} & {68.65} & {61.40} & {57.00} & {53.90} & {66.95} & - & - \\
\small\texttt{16} & MMT + ConCAT   & BT & \ding{51} & \texttt{RQI} & \textbf{68.62} & \textbf{61.42} & \textbf{57.08} & \textbf{53.99} & \textbf{66.98} & {69.80} & \textbf{70.00} \\

\midrule
 \small\texttt{17} & MMT + ConCAT + Triplet Loss~\cite{free_vqa}  & BT & \xmark & \texttt{RQI}& 68.11 & 60.70 & 56.23 & 53.10 & 66.59 & - & - \\  
 \band \small\texttt{18} & MMT + (SCL $\rightarrow$ CE)~\cite{Khosla2020SupervisedCL}  & BT & \xmark & \texttt{RQI}& 28.36 & 28.36 & 28.36 & 28.36 & 24.04 & 25.70 & - \\
 \small\texttt{19} & MMT + (CE + SCL w/ SCL batches) & BT & \ding{51} & \texttt{RQI} & 66.95 & 59.70 & 55.32 & 52.20 & 65.10 & 66.73 & - \\
  \band  \small\texttt{20} & MMT + (CE + SCL w/ Random batches) & BT & \ding{51} & \texttt{RQI} & 67.22 & 59.92 & 55.54 & 52.43 & 65.57 & 67.13 & - \\
 \small\texttt{21} & MMT + (CE + SCL w/ Joint backward) & BT & \ding{51} & \texttt{RQI} & 67.75 & 60.79 & 56.59 & 53.63 & 66.23 & - & - \\
 \band\small\texttt{21} & MMT + ConCAT + Dyn. Scaling (re-run) & BT & \ding{51} & \texttt{RQI} & 68.60 & 61.38 & 57.01 & 53.92 & 66.95 & - & - \\
\bottomrule

\end{tabular}
  \caption{\textbf{Evaluation on VQA-Rephrasings and VQA 2.0 dataset}. \textbf{DA} denotes the source of augmented data from either Back Translation (BT) or Visual Question Generation (VQG). \textbf{N-Type} defines the type of negatives used from Image (\texttt{I}), Question (\texttt{Q}) and Random (\texttt{R}). \textbf{Scaling} denotes whether scaling factor $\alpha$ (defined in Eq.~\ref{eq:alpha}) was used. When reporting on test-dev and test-std we train our model on train+val set of VQA 2.0 dataset.}
  \label{robustness_table}
\end{table*}



